Adversarially learning disentangled speech representations for robust multi-factor voice conversion

Factorizing speech as disentangled speech representations is vital to achieve highly controllable style transfer in voice conversion (VC). Conventional speech representation learning methods in VC only factorize speech as speaker and content, lacking controllability on other prosody-related factors. State-of-the-art speech representation learning methods for more speechfactors are using primary disentangle algorithms such as random resampling and ad-hoc bottleneck layer size adjustment,which however is hard to ensure robust speech representationdisentanglement. To increase the robustness of highly controllable style transfer on multiple factors in VC, we propose a disentangled speech representation learning framework based on adversarial learning. Four speech representations characterizing content, timbre, rhythm and pitch are extracted, and further disentangled by an adversarial Mask-And-Predict (MAP)network inspired by BERT. The adversarial network is used tominimize the correlations between the speech representations,by randomly masking and predicting one of the representationsfrom the others. Experimental results show that the proposedframework significantly improves the robustness of VC on multiple factors by increasing the speech quality MOS from 2.79 to3.30 and decreasing the MCD from 3.89 to 3.58.

==> backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% equation 公式 %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\ref{eq:decom})


${E} \in  \mathbb{R}^{N \times D}$


\begin{equation}
\small
\label{eq:bnm}
\mathcal{L}_{bnm} = - \frac{1}{N} {\| \mathbf{E}  \|}_{*}.
\end{equation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% figure 图 %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[htb]

\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=8.5cm]{image1}}
%  \vspace{2.0cm}
  \centerline{(a) Result 1}\medskip
\end{minipage}
%
\begin{minipage}[b]{.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image3}}
%  \vspace{1.5cm}
  \centerline{(b) Results 3}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image4}}
%  \vspace{1.5cm}
  \centerline{(c) Result 4}\medskip
\end{minipage}
%
\caption{Example of placing a figure with experimental results.}
\label{fig:res}
%
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% table 表格 %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% 最前面加引用  \usepackage{booktabs}
\begin{table}[!htb]
\renewcommand{\arraystretch}{1.3}
\caption{MOS and ANOVA comparison between WRF and proposed approach.}
\label{table:mos}
\centering
\begin{tabular}{c|r|r}
    \toprule
    Methods & WRF & Proposed\\ \midrule
            MCD & $0.946$ & $21.1\%$ \\ 
            MOS & $0.932$ & $20.8\%$ \\ 
    \bottomrule
 \end{tabular}
\end{table}


==> confusion.tex <==
% \begin{figure*}[t]
% 	\centering
% 	\hfill
% 	\begin{minipage}[b]{0.25\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figure/cossim.jpg}
% 		(a) Confusion matrix for speaker classification results of
% Speaker 1 synthesized samples.
% 	\end{minipage}
% 	\hfill
%     \caption{\textit{Cos similarity.}}
% 	\label{fig:cossim}
% \end{figure*}


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figure/cossim.jpg}
%   \caption{\textit{Cos similarity.}}
%   \label{fig:cossim}
% \end{figure}


\begin{figure}
\begin{minipage}{0.48\linewidth}
  \centerline{\includegraphics[width=3.0cm,height=3cm]{figure/baseline_nofre.png}}
  \centerline{(a) Baseline system}
\end{minipage}
\begin{minipage}{0.48\linewidth}
  \centerline{\includegraphics[width=2.95cm,height=3cm]{figure/proposed_nofre.png}}
  \centerline{(b) Proposed system}
\end{minipage}
\hfill
\caption{\textit{Normalized histogram of similarity values between utterances. The blue denotes same speaker and the orange denotes  different speakers.}}
\label{fig:cossim}
\end{figure}







==> content/0_abstract_backup.tex <==
\begin{abstract}
Factorizing speech as disentangled speech representations
%The disentanglement of speech representations
is vital to achieve highly controllable style transfer in voice conversion (VC).
Conventional speech representation learning methods in VC only factorize
speech as speaker and content, lacking controllability on other prosody-related factors. 
State-of-the-art speech representation learning methods for more speech factors 
%%%HINT: strategy/algorithm/method/mechanism
are using primary disentangle algorithms such as
random resampling and 
ad-hoc bottleneck layer size adjustment,
which however is hard to ensure robust speech representation disentanglement.
To increase the robustness of highly controllable
style transfer on multiple factors in VC,
we propose a disentangled speech representation learning framework based on 
adversarial learning.
Four speech representations characterizing 
content, timbre, rhythm and pitch are extracted,
and further disentangled by an adversarial network inspired by BERT.
The adversarial network is used to minimize the correlations between the speech representations, by randomly masking and predicting one of the representations from the others.
We adopt the Mel-GAN vocoder which greatly speeds up the inference speed.
Experimental results show that the proposed framework significantly improves the robustness of VC on multiple factors by increasing the speech quality MOS from 2.94 to 3.47 and decreasing the MCD from 3.89 to 3.58.


\end{abstract}

==> content/detailed.tex <==
\begin{figure*}[t]
	\centering
	\hfill
% 	\begin{minipage}[b]{0.65\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figure/a.png}
% 		(a) Overall architecture 
% 	\end{minipage}
% 	\hfill
	
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/b.png}\\\ \\  
		(a) gumbel-softmax
	\end{minipage}
	\hfill

	
    \begin{minipage}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/interspeech21.png}\\\ \\  
        (b) Mask-And-Predict
    \end{minipage}
    \hfill


	\caption{\textit{Architecture of the proposed multiple factor voice conversion system with adversarially disentangled speech representation learning.}}
	\label{fig:structure}
\end{figure*}


==> table/ABX.tex <==
\begin{table}[h]
	\caption{ABX comparison between proposed and baseline approaches.
	PR refers to preference rate.}
	\label{tab:ABX}
	\centering
	\begin{tabular}{lccc}
		\toprule
		 &\textbf{Baseline}  &\textbf{Proposed}
		 &\textbf{Neutral}\\
% 		 &\textbf{NP}\\
		\midrule
% 		\bottomrule
% 	Rhythm only &33.3\% &33.3\% &33.4\%
	 PR &20.6\%  &51.8\% &27.6\% \\
% 	 PR &10.7\% &34.5\% &29.8\% &25.0\% \\
% &\textbf{\%}\\
% 	Pitch only	&0\% &12.5\% &30\% \\
% % 	&\textbf{40\%}\\
% 	Timbre only	&75\% &25\% &75\% \\
% % 	&\textbf{40\%}\\
% 	Rhythm \& Pitch &37.5\% &25\% &50\% \\
% % 	&\textbf{40\%}\\
% 	Rhythm \& Timbre  &62.5\% &37.5\% &55\% \\
% % 	&\textbf{40\%}\\
% 	Pitch \& Timbre &62.5\% &25\% &80\% \\
% % 	&\textbf{40\%}\\
% 	All &75\% &25\% &75\% \\
% 	&\textbf{40\%}\\
% 		\midrule
% 		&\textbf{No Preference} &\textbf{Baseline} &\textbf{Finetuned Baseline}&\textbf{Proposed}\\
		\bottomrule
	\end{tabular}
\end{table}

==> table/ablation.tex <==
\begin{table}[ht]
	\caption{Effect of Word prediction network on reconstruction loss and adversarial loss reduction.
% 	Baseline+ refers to the speechflow with finetuned sizes of bottlenecks.
	}
	\label{tab:Ablation}
	\centering
	\begin{tabular}{lccc}
		\toprule
		 &\textbf{Proposed with} &\textbf{Proposed-without}\\
		 &\textbf{word prediction}
		 &\textbf{word prediction}\\
		\midrule
% 		\bottomrule
		Reconstruction loss &\textbf{12.8} &21.5\\
		Adversarial loss &\textbf{0.015} &0.016\\
% 		Adversarial loss	&0 &0 &30\%	&\textbf{40\%}\\
% 		Timbre-only	&10\% &20\% &30\%	&\textbf{40\%}\\
% 		\midrule
% 		&\textbf{No Preference} &\textbf{Baseline} &\textbf{Finetuned Baseline}&\textbf{Proposed}\\
		\bottomrule
	\end{tabular}
\end{table}

==> table/conversion_rate.tex <==
% \begin{table}[h]
% 	\caption{MCD comparison between different approaches. 
% % 	Baseline+ refers to the speechflow with finetuned sizes of bottlenecks.
% % 	, baseline and fine-tuned baseline approaches.
% 	}
% 	\label{tab:MCD}
% 	\centering
% 	\begin{tabular}{lcc}
% 		\toprule
% 			&\textbf{Baseline} &\textbf{Proposed}\\
% 		\midrule
% 		MCD &4.00	&3.94\\
% 		\bottomrule
% 	\end{tabular}
% \end{table}


% \begin{table}[h]
% 	\caption{Objective evaluation results on systems.
% 	}
% 	\label{tab:Objective}
% 	\centering
% 	\begin{tabular}{lcc}
% 		\toprule
% 		 &\textbf{MCD} &\textbf{RCA}\\
% 		\midrule
% 		baseline &4.00 &0.629\\
% 		+ discrete rhythm code &3.96 &0.630 \\
% 		+ MAP &3.83 &0.780 \\

% 		\bottomrule
% 	\end{tabular}
% \end{table}

%%%%%%%% %%%%%%%% 
% 以下为完全不报错、且格式正确、内容暂时正确的表格
% \begin{table}[h]
% 	\caption{Objective results performed over 100 utterances of les than 5 seconds from the test partition. The reported values are the mean and the standard deviation of the sample. First three FastVC variants are described later in Section 5.3.
% 	}
% 	\label{tab:Objective}
% 	\centering
% \begin{tabular}{lll}
% \hline Experiment &Training data &MCD\\
% \hline SpeechFlow\cite{qian_auspicious3000speechsplit_2020} &train20 & $\mathbf{2.56 \pm 0.23}$ \\
% &train107 &\\
% &train303 &\\
% \hline Spk-emb &train303 & $2.57 \pm 0.25$ \\
% D-R &train303 & $2.57 \pm 0.25$ \\
% % posed in [6] & \\
% \hline D-R+MAP &train20 & $2.61 \pm 0.24$ \\
% &train107 &\\
% &train303 &\\
% % FastVC with  & $2.62 \pm 0.24$ \\
% % FastVC  & $\mathbf{2 . 6 8 \pm 0 . 2 2}$ \\
% % \hline FastVC w& $1.56 \pm 0.29$ \\
% % FastVC wit & $1.50 \pm 0.40$ \\
% % PhonetVC  & $\mathbf{1 . 6 7 \pm 0 . 3 0}$ \\
% \hline
% \end{tabular} 
% \end{table}


\begin{table}[h]
	\caption{\textit{Conversion rate on different speech factors of two systems.}
	}
	\label{tab:Objective}
	\centering
\begin{tabular}{llll}
\hline  &Rhythm &Pitch &Timbre\\
\hline Baseline\cite{qian_auspicious3000speechsplit_2020} &63.6 &15.2 &75.8 \\
Proposed &54.6  &48.5  &54.5 \\
\hline
\end{tabular} 
\end{table}

==> table/gender.tex <==
\begin{table}[h]
	\caption{\textit{The Similarity MOS for conversion between different combinations of gender.
	The ``BS'' denotes the baseline system and ``PP'' denotes the proposed one.}
	}
	\label{tab:gender}
	\centering
	\begin{tabular}{lcccc}
		\toprule
		 &\textbf{F-F}  &\textbf{F-M}
		 &\textbf{M-M} &\textbf{M-F}\\
		\midrule
	 BS &$3.79\pm0.11$  &$3.79\pm0.11$ &$3.79\pm0.11$ &$3.79\pm0.11$\\ 
	 PP &$3.79\pm0.11$  &$3.79\pm0.11$ &$3.79\pm0.11$ &$3.79\pm0.11$\\
		\bottomrule
	\end{tabular}
\end{table}

==> title.tex <==
% \title{speech representation learning for robust multi-factor voice conversion}%
% \title{Disentangled Speech Representation Learning via Adversarial Network for Robust Multi-Factor Voice Conversion}%
\title{Adversarially learning disentangled speech representations for robust multi-factor voice conversion}%
% \title{Improving  voice conversion system with adversarial learning for speech representation disentanglement by Mask-And-Predict}%
% adversarial 
% disentangle
\name{Jie Wang$^{1, \dagger}$,
\thanks{$\dagger$ Work performed while interning at Huya Inc.}
        Jingbei Li$^1$,
        Xintao Zhao$^1$,
       Zhiyong Wu$^{1,3,\ddagger}$,
% }
\thanks{
$\ddagger$ Corresponding author.}, Shiyin Kang$^2$, Helen Meng$^{1,3}$}
% \address{Author Affiliation(s)}
% \thanks{$\dagger$ Work performed during an internship at Huya Inc.}
% \thanks{
% $\ddagger$ Corresponding author.}, Helen Meng$^{1,3}$}
\address{
    % $^1$ Shenzhen International Graduate School, Tsinghua University, Shenzhen, China\\
    % $^2$ Department of Systems Engineering and Engineering Management, \\The Chinese University of Hong Kong, Hong Kong SAR, China\\
    $^1$ Tsinghua-CUHK Joint Research Center for Media Sciences, Technologies and Systems, \\
Shenzhen International Graduate School, Tsinghua University, Shenzhen, China\\
$^2$ Huya Inc, Guangzhou, China\\
$^3$ Department of Systems Engineering and Engineering Management, \\ The Chinese University of Hong Kong, Hong Kong SAR, China\\
    \small{\{jie-wang19,lijb19,zxt20\}@mails.tsinghua.edu.cn,
    kangshiyin@huya.com
	\{zywu,	hmmeng\}@se.cuhk.edu.hk}
    }
% \email{
% 	\{jb-li15, lirn15\}@mails.tsinghua.edu.cn,
% 	zywu@sz.tsinghua.edu.cn\\
% 	\{zhipengpeng, yangsong1\}@100tal.com,
% 	hmmeng@se.cuhk.edu.hk
% }
\maketitle
